Regaining Trust: Impact of Transparent User Interface Design on Acceptance of Camera-Based In-Car Health Monitoring Systems

Introducing in-car health monitoring systems offers substantial potential to improve driver safety. However, camera-based sensing technologies introduce significant privacy concerns. This study investigates the impact of transparent user interface design on user acceptance of these systems. We conducted an online study with 42 participants using prototypes varying in transparency, choice, and deception levels. The prototypes included three onboarding designs: (1) a traditional Terms and Conditions text, (2) a Business Nudge design that subtly encouraged users to accept default data-sharing options, and (3) a Transparent Walk-Through that provided clear, step-by-step explanations of data use and privacy policies. Our findings indicate that transparent design significantly affects user experience measures, including perceived creepiness, trust in data use, and trustworthiness of content. Transparent onboarding processes enhanced user experience and trust without significantly increasing onboarding time. These findings offer practical guidance for designing user-friendly and privacy-respecting in-car health monitoring systems.

==> body.tex <==

\section{Introduction}
In recent years, there is growing interest in integrating health monitoring systems into cars to provide real-time monitoring and support for individuals with chronic health conditions. These systems commonly utilize camera-based technologies to capture vital health information to enhance driver safety by detecting health emergencies in real-time and alerting emergency services. %Even if the potential benefit of such systems are apparent, it is crucial to understand how users perceive and interact with such systems to ensure their acceptance and effectiveness.

This study investigates the impact of transparent user interface design and camera-based health monitoring systems on users' experience and acceptance. We address two primary research questions:

\researchq{RQ1}{How does transparent user interface design impact users' experience of a health monitoring system?}

\researchq{RQ2}{Do users with health conditions have aversions to camera based health monitoring systems in cars?}

In this paper, we present our methodology for investigating these questions, including the study design, participant recruitment, and our data collection procedure. We describe the design of the interactive online prototypes, along with the measures employed to assess user perception and experience. Furthermore, we outline the data analysis approach and statistical tests used to examine the hypotheses.
\input{fig_proto_live}

The findings from this study contribute to a more comprehensive understanding of user acceptance and experience of camera-based health monitoring systems in cars. These insights can inform the design and implementation of transparent user interfaces that more effectively support users' needs and preferences.

\section{Related Work} 

\subsection{The Privacy Hump in Technology Acceptance}

The adoption of new technologies, particularly those that are potentially intrusive, often faces a ``privacy hump''. This term, as defined by \citet{EndUserPrivacyHCI}, refers to initial resistance or concerns that users may have about their privacy when they first encounter a new technology. Such concerns can stem from both misunderstandings about the technology, or other legitimate concerns about its use.

In the early stages of a technology's lifecycle, the privacy hump can pose a significant barrier to its acceptance. Users may be wary of how the technology will be used, and businesses may struggle to communicate the benefits of the technology effectively. Further, such concerns are commonly abstracted under umbrella terms of ``privacy'' or ``invasiveness''.

However, as the technology matures and its value proposition becomes clearer, the privacy hump tends to diminish~\cite{LongSurveillance}. The worst fears about the technology often do not materialize, and society adapts to its presence. Simultaneously, legal measures may be put in place to protect users' privacy and penalize violations, further alleviating privacy concerns.

In the context of in-car camera-based health monitoring systems, the privacy hump is a crucial factor. Given the potentially intrusive nature of these systems, users may initially have significant privacy concerns. Prior work suggests that strategies such as transparent user interface design and appropriate onboarding could be effective in addressing these concerns, making the system's operations and data usage clear to users. However, the effectiveness of these strategies in overcoming the privacy hump for in-car camera-based health monitoring systems warrants further exploration.

An alternative concept that may more accurately describe the ``feeling'' of the privacy hump is ``creepiness''. This term, as used in the field of Human-Computer Interaction (HCI), refers to the unsettling feeling that users may experience when interacting with a technology~\cite{Langer2018-po, Seberger2022-pt,Tene2013-nj}. %The concept of creepiness has been operationalized in the Creepiness Rating Scale (CRoSS), which measures emotional creepiness and creepy ambiguity~\cite{Langer2018-po}. %The scale was inspired by previous work by \citet{Seberger2022-pt} and \citet{Tene2013-nj}. It has been found to correlate positively with privacy concerns and computer anxiety, but negatively with controllability and transparency~\cite{Langer2018-po}.% This suggests that addressing the feeling of creepiness could be a key strategy in overcoming the privacy hump.

\subsection{Privacy Preserving Technology}

In response to privacy concerns associated with camera-based sensing, alternative sensors have been explored by commercial entities~\cite{Lien2016-qt}. For instance, radar sensors can detect movement and gestures without capturing detailed visual information, potentially making them more acceptable to users.

Efforts have also been made to improve the performance of these alternative sensors. A study by \citeauthor{Vid2Doppler} used video data to train machine learning algorithms for mmWave sensing, aiming to offer similar activity tracking as cameras but without the privacy implications \cite{Vid2Doppler}.

Additionally, modifying the camera output, such as applying a Gaussian blur filter, can strike a balance between awareness and privacy \cite{FiltersAwarnessPrivacy}. Various visual privacy protection approaches, including pixelation, blurring, and avatar replacement, can also be applied to reduce perceived invasiveness \cite{VisualPrivacyProtectionSurvey}.

New approaches to data based machine learning attempt to ease privacy concerns. %Some of them appear particularly suitable in the automotive health sensing context. 
Among them are differential privacy \cite{nelson2017introducing}, federated learning and homomorphic encryption \cite{pandey2022introduction}. While these alternatives show promise, their effectiveness in reducing privacy concerns and increasing user acceptance in the context of in-car health monitoring systems still requires further exploration~\cite{10.1145/3411764.3445677, Saleem_2018}. 

% \subsection{Health Monitoring in Cars}

%Contextual integrity
\subsection{Contextual Integrity (CI) vs Privacy Perceptions}

The theory of CI provides a nuanced perspective on privacy, challenging the conventional public-private dichotomy often found in privacy literature~\cite{PrivacyInContextNissenbaum}. According to Nissenbaum, privacy should not be viewed as a matter of information control, but rather as appropriate information flow within specific contexts. Under this framework, norms are clearly defined by the information’s subject, sender, recipient, type, and transmission principles. The CI framework determines the appropriateness of information flows that align with societal values and ethics within specific contexts.% In other words, whether a particular flow of information is deemed appropriate or not depends on the context, the nature of the information, and the parties involved. CI recognizes that societal norms and expectations can significantly influence perceptions of privacy.

There can be a disconnect between end-user perceptions of privacy and the normatively appropriate flow of information as defined by CI. Users may have privacy expectations or concerns that do not align with the norms of information flow within a particular context. This disconnect can be especially pronounced in the context of new technologies, such as in-car camera-based health monitoring systems, where societal norms and expectations are still formalizing \cite{PrivacyInContextDoyle}.

% Understanding and addressing this disconnect is crucial for the design and acceptance of such systems. Transparent user interface design, for instance, can help bridge this gap by making the system's operations and data usage clear to users, thereby aligning user perceptions with the normatively appropriate flow of information.

Importantly, CI evaluates the appropriateness of information flow, not only by the information that is recorded by, for example, a sensor, but by the attribute that is transferred. With the advent of AI inference, these attributes, such as one's eye blinking rate, are sensor-independent. This means that the privacy implications of a technology are not necessarily tied to it, but rather to the information it infers and transfers \cite{Barkhuus2012-sz, Apthorpe2018-qd}.% This further underscores the importance of considering the context and the nature of the information flow in evaluating the privacy implications of in-car camera-based health monitoring systems.

\subsection{Transparency and Explainability}
The digitization of the car poses new challenges and approaches to user experience design. \citet{10.1145/3543174.3546846} show that artificial intelligence in vehicles requires explanations to foster perceived understandability and transparency of the system, however, insufficiently designed explanations can decrease acceptance of the system. The need for explanation can be in conflict with shareholder interests, and businesses may be inclined to nudge users towards commercial interests through deceptive explanations, control and transparency~\cite{Chromik2019DarkPO}.% Whether users notice business nudging them to their preferred choice through lack of detailed explanation is still an under-explored area. 

\subsection{Privacy Policies and Terms of Use}

Terms of Use outline the rules, rights, and responsibilities that users agree to when accessing applications or services. Typically, these terms cover user conduct, intellectual property rights, disclaimers, limitations, and mechanisms to resolve disputes. Terms of Use create a contractual agreement between an individual and the service provider \cite{lemley2006terms}. While Terms of Use govern the user's conduct and responsibilities, privacy policies address the collection, use, and protection of personal information. Privacy policies are a fundamental part of a Terms of Use agreement \cite{steinfeld2016agree}.

Prior work on privacy policies suggest that they can obscure crucial information that would otherwise help data subjects form norms about their privacy in novel technologies. Specifically, when privacy policies elide key contextual information, data subjects resort to drawing on their own imagination, distorting the milieu entirely \cite{martin2016measuring}. 

Privacy policies also suffer from ambiguity and complexity, pointing to a growing tension between legal compliance and business interests. Such policies are often drafted to legally protect organizational interests, while also maximizing their ability to collect and utilize data. As a result, language used in privacy policies can be convoluted and difficult for individuals to follow, creating a barrier for informed decision-making. % One way to remedy this challenge is to enact comprehensive and enforceable privacy regulations that establish clear standards for transparent, concise, and meaningful privacy policies.

%Other popular privacy policy models, such as notice and consent statements, reduce participation down to a choice where the risks of agreement or disagreement are poorly defined \cite{barocas2009notice}. The inadequacies of ‘notice and consent’ can be traced to (1) a disconnect between the policies of the platform and the policies of the third parties they contract, (2) the changing nature of privacy policies, and (3) the ubiquitous nexus of participants in novel technological domains. Both Terms of Use and privacy policies play a vital role in setting expectations and establishing a legal framework for users' interactions.  

\subsection{Regulatory Mechanisms and Their Failures}

The General Data Protection Regulation (GDPR) enhances data protection and privacy for individuals within the European Union (EU)~\cite{jones2020american}. It mandates organizations to justify their data processing activities, facilitating GDPR compliance \cite{goddard2017eu}. The GDPR empowers individuals to control their personal data, redressing the power imbalance between data subjects and data processors.

In the context of GDPR, dark patterns have emerged as a concern. Dark patterns are design techniques that manipulate user behavior, often exploiting cognitive biases and manipulative tactics to nudge users towards actions benefiting the platform or organization, potentially infringing on privacy rights \cite{gray2018dark}. Dark patterns can involve deceptive interface elements that coerce users into sharing more personal data.
% The General Data Protection Regulation (GDPR) focuses on data protection and privacy for individuals within the European Union uu(EU)~\cite{jones2020american}.Along these lines, the GDPR mandates organizations to identify and justify legal grounds for their data processing activities, of which consent is one option among several. By aligning data processing practices with lawful grounds, organizations can more effectively navigate GDPR compliance \cite{goddard2017eu}.The GDPR further confers fundamental rights to individuals by empowering them to exercise control over their personal data. This creates opportunities for individuals to assert their autonomy and redress the existing power imbalance between data subjects and data processors. 

% Enacted in 2018, the GDPR supersedes EU's prior Data Protection Directive and harmonizes data protection laws across EU member states. The GDPR's core objective is to endow individuals with enhanced control over their personal data, while imposing strict obligations on organizations, both domestic and international, who are involved in the processing EU residents' personal information \cite{goddard2017eu}.

% These rights include, but are not limited to the right to access personal data held by organizations, the right to restrict data processing, and the right to data portability. 

% Within the context of the GDPR and enhanced regulatory compliance, the relationship between dark patterns and UX design has emerged as a concerning phenomenon. Dark patterns are deliberate interface design techniques that manipulate user behavior towards making decisions. These design patterns often exploit cognitive biases, information asymmetry, and manipulative tactics to nudge users towards actions that benefit the platform or organization, while potentially infringing on individuals' privacy rights \cite{gray2018dark}. Dark patterns can involve deceptive interface elements such as buttons, confusing options, hidden defaults, or misleading language that coerce users into sharing more personal data. %Further, these practices nudge users towards sharing more personal data than intended, granting excessive permissions, or unknowingly subscribing to services. 

\section{Methodology}
\subsection{Study Design}
% Details of the study design, like the nature of the experiment, the use of control and experimental groups, etc.

In this study, we gathered data from online participants rather than conducting experiments in a laboratory setting. This approach was crucial in order to acquire more diverse and representative data that considers the range of health conditions reported by our participants. Health conditions can influence how and when participants are able to interact with the study materials, and an online setting provides the flexibility needed to accommodate these individual needs.
As \citet{Clifford2014-hu} state, there are minimal differences between online and lab-based participants in terms of the level of attention and socially desirable responding. Specifically, that online participants tend to consult outside sources. However, this concern is not relevant to our study, which investigates perceptual user experience dimensions. 
To further ensure the validity of our data and limit the potential influence of distractions common in online settings, we implemented several countermeasures. These include strategies such as clear instructions, time restrictions on tasks, and attention checks throughout the study.
%This approach allows us to gather meaningful and representative data, while also accommodating the needs of our participants, particularly those with health conditions.

% Maybe the first part of this in the methods section and the rest in the discussion? 
% Maybe a few sentences here / somewhere about how we consider CI / blending Terms of Use and privacy policies / and dark patterns in the design of the onboarding prototypes. and maybe in the discussion we have a short paragraph about how there isn't aversion because the flow is appropriate / clear. we can add like a little CI analysis spelling out the CI tuple: information’s subject (user / participant), sender ( x ), recipient ( x ), type ( x ) , and transmission principles ( x )

A total of 42 participants were recruited for this study, including a pilot of the study with 12 participants. The recruitment was conducted using Prolific (\url{www.prolific.co}), with a focus on achieving a balanced and diverse sample from the U.S. Out of the 42 participants, 40 provided demographic information.

The participants' ages ranged from 20 to 75 years, with an average age of approximately 41 years and a standard deviation of 14.84, indicating a fairly even distribution across the age spectrum. The gender distribution was also balanced, with 19 females and 21 males. The majority of the participants were White (33 out of 40). All participants were U.S. citizens, although 4 were born outside the U.S.

The study aimed to include participants who regularly drive a car and have a long-term health condition or disability. These criteria were verified through screener questions in our survey. The health conditions reported by the participants varied widely, with several participants having more than one condition. The most common condition was diabetes, reported by 18 participants. Heart conditions were reported by 10 participants, mental health conditions by 4 participants, and epilepsy by 2 participants. All other conditions were not reported more than once. %Those were ME/CFS, Behet's Syndrome, Irritable Bowel Syndrome, Chronic Pain, Anal Fissure, Asthma, Chronic Kidney Disease (CKD), Dry Eye Disease, Dwarfism, Hypoglycemia, and Waldenstrom Macroglobulinemia.


\subsection{Hypotheses}
We expect that the prototype conditions, which vary in designed information transparency, interface deception, choice and information complexity, as well as visualization, will affect the user evaluation in the following ways:

\hypothesisShort{H1} Perceived Creepiness will be lowest with a detailed Onboarding flow and lower with a blurred camera view.
\hypothesisShort{H2} User Experience with a transparently designed Onboarding procedure will be the highest.
\hypothesisShort{H3} Trust in Data Use and Trusworthiness of Content will be the highest with a transparently designed Onboarding procedure, and lowest with Deceptive user interface design. 
\hypothesisShort{H4} Usability will not be significantly affected by the type of Live View Camera Feedback. 
\hypothesisShort{H5} Hedonic Quality will be higher with Live View Camera Feedback than without.
\hypothesisShort{H6} Trust in the Data Use and Trusworthiness of Content will be affected by the Live View Camera Feedback.
\hypothesisShort{H7} Users will not spend more time reading Terms and Use than in the other conditions. 


\subsection{Procedure}

42 car users with chronic health conditions engaged in an online experiment where they interacted with two prototypes in 6 conditions hosted online. After interacting, and observing each prototype condition, participants were asked to complete a series of questionnaires. These questions measured the perceived user experience using 7-point Likert scales. The order of prototype conditions was randomized. Participants were paid \$2.60  which amounts to \$11.64/hr on average for the study which took a median time of 13:24 minutes. The time spent assessing each prototype was measured. 

\subsection{Materials and Instruments}
The study focused on the impacts of onboarding, including terms of use and privacy policy, and Live View, including real-time monitoring feedback. Mockups were created with Apple Freeform, and refined over two weeks with input from a health monitoring software company, and translated into semi-functional online prototypes using Framer~\cite{Framer_2022}. %The tool simplifies design and development of interactive web apps and supports complex JavaScript React code through custom code overrides and components. 

The onboarding requires the user to accept or decline the Terms of Use of the technology, and to decide whether they want to share data with the technology provider. 
Three designs were used: The first is a state-of the art condition which does provide typical Terms of Use \textit{(T\&U)} based user onboarding in the format of legal text. The second design employs deceptive designs \cite{Gray2023-ei}) to nudge users to accepting the default business preferred options \textit{(Business Nudge)}. The third option uses a multi-step onboarding process, explaining in chunks what the user agrees to and the options they have \textit{(Transparent Choice)}. Final designs of all onboarding conditions were reviewed by legal professionals. 

The live view prototype conditions differed in the live camera feedback. Each showed the same simulated Health sensing parameters: once without any camera feedback \textit{(No Camera)}, once showing the live camera feed of the participant, overlaid with a mesh of facial landmarks \textit{(Camera View)}, and once showing the blurred live camera feed of the participant, overlaid with a mesh of facial landmarks \textit{(Blurred Camera)}.

% \subsection{Design Considerations} %placeholder (AI expanded text)

% -> needs to be moved to text above

% In designing the onboarding prototypes, we drew upon CI to create an onboarding process that ensures appropriate information flow and respects the privacy norms of this novel context. This involved clearly defining the CI tuple: the information’s subject (user/participant), sender (the health monitoring system), recipient (healthcare provider or system), type (health data), and transmission principles (consent-based, with clear disclosure and option to opt-out).

% In an effort to prioritize transparency and user-friendliness, the language in our Terms of Use includes our privacy policies. We avoided complex legal jargon and presented information in a clear and concise manner. Finally, we were mindful of the potential for dark patterns in the design process 

\input{fig_proto_onboarding}
To enhance realism, the prototype was embedded in a virtual cockpit screen, complete with an animated road and steering wheel. Subtle animations, randomized health sensing text and vehicle speed, and scrolling effects and transitions were included. The Google Media Pipe Facemesh model was used for animating the facemesh, ensuring performance and accuracy across diverse populations\footnote{\url{https://www.npmjs.com/package/@tensorflow-models/face-landmarks-detection}}~\cite{Kartynnik2019-ij}.

\subsection{Measures}

Five scales were used in the study, each assessing different aspects of user perception and experience:
\textit{}{Pragmatic Quality}: This scale, as part of the User Experience Questionnaire (UEQ), assesses the perceived usability of the technology and its user interface. 
\textit{Hedonic Quality}: This scale, as part of the UEQ, evaluates the stimulation and novelty of the technology and its user interface~\cite{Schrepp2017-tl}.
\textit{Creepiness}: This scale assesses the degree to which participants find the technology unsettling. It contains three items, each rated on a 7 point Likert scale. The creepiness scale was inspired by work by \citet{Seberger2022-pt, Tene2013-nj} and the CRoSS scale~\cite{Langer2018-po}.
\textit{Trustworthy Content}: This scale, as part of the modular UEQ extension, evaluates the perceived usefulness and trustworthiness of the information provided by the product~\cite{Schrepp2019-dq}.
\textit{Data Use (Trust)}: This scale, as part of the modular UEQ extension, measures the perceived security and reliability of the product's use of personal data~\cite{Hinderks2016-tv}. All UEQ and UEQ extension scales were 7 point bipolar Likert scales. The exact subscale text can be found in the appendix \autoref{tab:scalereliability}.

\subsection{Data Analysis}
\subsubsection{Factorial Reliability}
Before conducting the full study, factorial reliability was calculated for each scale using Cronbach's alpha using Jamovis factorial analysis package~\cite{csahin2019jamovi}. This measure was used to assess the internal consistency of the scales. The Cronbach's alpha values for all scales were above the commonly accepted threshold of 0.7, indicating a high level of internal consistency for each scale. Specifically, the Creepy scale, which is not a validated scale and was created for this study, had a Cronbach's alpha of 0.96. The mean scores, standard deviations and Cronbach's alpha values can be found in the appendix \autoref{tab:scalereliability}.
\setlength{\parskip}{-5pt}

\subsubsection{Data Inclusion}
No completed responses were omitted from inclusion, and data was minimally cleaned for analysis. No participants completed the survey unreasonably fast (less than half the median time). Two participants timed out, however, after assessing their data, it was chosen to include their response. Two responses had missing data points, and one response showed straightlining for the sub-scale items. The limited missing items and no detection of straightlining indicate general good data quality.

\subsubsection{Statistical Analysis}
Data was analyzed using R Studio. For the statistical analysis, we first inspected the normality and homogeneity of variance assumptions using Shapiro-Wilk and Levene's tests, respectively. Depending on the results of these tests, either parametric or non-parametric tests were conducted to analyze the data. 
Descriptive statistics, including mean scores, standard deviations, p values and effect sizes, were computed for each scale. In addition to the statistical analysis, violin plots were created with the ggplot2 and ggstatsplot package\footnote{\url{https://github.com/IndrajeetPatil/ggstatsplot}} for R. Initial data analysis was also conducted using the UEQ Excel analysis tools\footnote{\url{https://www.ueq-online.org/}}; these are not reported here. The violin plots were zeroed (-3 to +3) so that common interpretations of the UEQ, such as interpreting values between -0.8 and 0.8 as neutral and outside as positive or negative can be made.

\setlength{\parskip}{0pt}

% The NPAV found a significant main effect of \Comparison on Trust (\F{2}{22}{5.44}, \p{0.012}). The NPAV found a significant interaction effect of \Comparison $\times$ \Prototype on Trust (\F{2}{22}{5.30}, \p{0.013}). 


% \onboarding  will be \liveview replaced with "Onboarding" in small caps, \deceptive will appear as bold, red text saying "Deceptive", etc. \transparent \stateoftheart \lvNocamera 

% \lvNoFacialLandmarks, \lvCameraView, \lvBlurredCameraView, \onbTermsConditions, \onbDetailedOnboarding,\onbBusinessDefaults





\section{Findings}

Our findings indicate that participants responded differently across the scales. Here, we present the results of the factorial reliability analysis and the descriptive statistics for each scale.


% \subsection{Descriptive Statistics} 

% The mean scores and standard deviations for each scale over all prototypes are presented in Table \ref{tab:scalereliability}. The mean score for the Creepy scale was -1.3, indicating that, on average, participants did not find the prototypes overly creepy. The mean score for the Trustworthy Content scale was 0.87, suggesting that participants slightly positively rank the prototypes. For the Data Use (Trust) scale, the mean score was 0.53, showing that participants on average neutrally evaluate the prototypes here. The Pragmatic Quality scale had a mean score of 1.3, indicating that participants rank the Usability of the prototypes positively. Finally, the mean score for the Hedonic Quality scale was 1.29, suggesting that participants rank the hedonic experience of the prototypes positively. 

\subsection{Statistical comparisons}
% Results from ANOVAs and pair-wise t-tests are presented in the violin plot figures. 
The hypotheses were analyzed using a combination of ANOVAs and pair-wise t-tests. The results of these statistical tests are visually represented in the violin plot figures, providing insights into the differences between the prototype conditions.

The hypothesis tests revealed significant findings on the impact of different design variations on user experience measures. The specific results and their interpretations are presented here briefly. 


\input{fig_violins_creep_time}
\input{fig_violins_onboarding}


% \begin{itemize}[label={},leftmargin=0pt]
%   \item \textbf{Creepiness:} The Transparent choice condition had the lowest perceived creepiness for the Onboarding prototype, while the Business nudge condition had the highest. The Blurred camera condition had the lowest perceived creepiness for the Live View prototype.
  
%   \item \textbf{Hedonic Quality:} The different design variations in the Onboarding prototype did not significantly impact Hedonic Quality.
  
%   \item \textbf{Pragmatic Quality:} The Terms and Conditions condition had the lowest perceived usability, while the Transparent choice condition had the highest perceived usability for the Onboarding prototype.
  
%   \item \textbf{Trust Data Use and Trustworthy Content:} The differences in Trust Data Use and Trustworthy Content for the Onboarding prototype were not significant. However, the effect sizes suggest potential meaningful differences with a larger sample size. In the Live View prototype, there were no significant differences in these measures.
  
%   \item \textbf{Time Spent Evaluating Prototype:} Participants spent less time on the Terms and Conditions condition compared to the other conditions for the Onboarding prototype. In the Live View prototype, participants spent more time on the Blurred camera condition compared to the No camera condition.
% \end{itemize}


% These findings offer insights into the impact of design variations on user experience measures. Please refer to the violin plots for detailed statistical tests and results.
\hypothesis{H1}{Accept} The results indicate that the Transparent Choice had the lowest perceived Creepiness in the Onboarding Prototype and that Blurred Camera had a lower perceived Creepiness than the Camera View, supporting the hypothesis.
\hypothesis{H2}{Accept}  Transparent Choice during Onboarding is preferred over the text heavy Terms and Conditions in both Hedonic and Pragmatic Qualities.
\hypothesis{H3}{Accept} Trust in Data Use and Trustworthiness of Content were significantly higher than with the simplified Business Nudge in the Onboarding. 
\hypothesis{H4}{Accept} The results indicate that there were no significant differences in perceived Usability (Hedonic Quality) between the Live View Camera Feedback conditions, supporting the hypothesis.
\hypothesis{H5}{Reject} There were no significant differences in Hedonic Quality between the conditions of the Live View. The mean of Hedonic Quality for Blurred Camera and Camera View were only marginally higher. 
\hypothesis{H6}{Reject} Trust in the Data Use was significantly affected by the Blurred Camera but only with a very small effect\footnote{\url{https://www.statisticshowto.com/omega-squared/}}. Trustworthiness of Content was not affected by the Live Camera View.
\hypothesis{H7}{Accept}  The results indicate that participants did not spent significantly more time on the Terms and Conditions condition compared to the other two conditions, supporting the hypothesis.


% \subsection{Non-parametric Analysis of Variance}

% The NPAV revealed significant main effects of the Onboarding prototype comparison on perceived creepiness, $F(2,22)=5.31, p=0.013$, as well as the Live View prototype comparison, $F(2,22)=5.56, p=0.011$. Moreover, there was a significant interaction effect between the comparison conditions and the type of prototype on perceived creepiness, $F(2,22)=8.79, p=0.002$.


% A significant main effect of the comparison condition on the timing of the last click on each prototype was also observed, $F(2,22)=6.12, p=0.008$. Additionally, there was a significant interaction effect between the comparison condition and the type of prototype on this timing, $F(2,22)=3.57, p=0.046$.

% The analysis revealed a significant main effect of the comparison condition on the perceived pragmatic quality of the onboarding process, $F(2,22)=3.67, p=0.042$.

% However, no significant effects of the comparison condition or the type of prototype were found on trust, trustworthiness, hedonic quality, or overall pragmatic quality.

The results of these analyses, along with the descriptive statistics and reliability coefficients, are visually represented in Figures \ref{fig:Creep}-\ref{fig:LastClicks}.

\section{Discussion}

Our study provides insights into the role of transparent design in shaping user perceptions of privacy and trust in the context of in-car camera-based health monitoring systems. The findings suggest that transparency in design can help to align user perceptions with the normatively appropriate flow of information, as defined by CI.

In particular, our results indicate that a transparently designed onboarding procedure with clear and concise terms and conditions can significantly enhance user experience and trust in data use. The multi-step onboarding with detailed and unavoidable explanations of terms of use and privacy policy, did not score worse on usability. This aligns with the existing literature on the inadequacies of ‘notice and consent’ and the need for more user-friendly and accessible privacy policies.
Finally the results indicate that users do not have aversions against health monitoring and cameras in cars per se, as shown by the non-negative assessment, across all measures and across all conditions, including those that follow the state of the art condition. 
This also aligns with the principles of CI, which emphasizes the importance of appropriate information flow over categorizing data sensitivity simply by type.  


% \begin{itemize}
% \item participants who find this creepy and not trustworthy / have concerns
% \item none of them were assessed negatively, overall there is no strong aversion  
% \end{itemize}


\section{Future work}
Our findings suggest that users do not exhibit aversion towards camera-based in-car health sensing. Furthermore, it demonstrates that intentional design choices can influence the perception of user experience. While the provided prototypes offer initial guidance, designing for a specific usage context and adhering to domain specific legislation require individualized design decisions.

%Our results indicate that prioritizing the design of the appropriate onboarding interface significantly impacts multiple measures. However, the design of the live view interface should not be entirely deprioritized. The trust in data use received lower ratings, and the presence of a blurry camera image could influence the perception of creepiness. Thus, both interfaces warrant careful consideration in the design process.

While our industry embedded study can contribute to better implementations of health sensing in the broader car industry, it also provides emerging generalizable evidence. A follow-up study should aim for a more systematic exploration of design options by altering individual dimensions in a controlled manner. In contrast to this study, where prototypes varied multiple design dimensions simultaneously, for example, focusing on individual dimensions such as transparency level, choice level, and deception level will allow for a more precise understanding of their individual impacts.

\section{Conclusion}

In this study, we investigated the impact of transparent design on user perceptions in the context of in-car camera-based health monitoring systems. Our findings suggest that transparent design can significantly enhance user perceptions of privacy and trust, and improve overall user experience. These findings will inform further research on design practices in this area, contributing to the development of more user-friendly and privacy-respecting data driven technologies.

%\subsection{Acknowledgements}
%We would like to thank [redacted for blind review] for providing their design requirements for the prototypes and supporting us in participant recruitment. We would also like to thank [redacted] for his willingness to run this study as a course project.

% \subsection{Necessary Sample Size for Follow-up Study}

% In our preliminary within-subjects study, an ANOVA was conducted to examine the effect of three Onboarding Prototypes - terms and conditions, transparent choice, and business nudge - on Trust in Data Use (see: \autoref{fig:OnboardingTrust} left). The sample size was 12, and the observed Fisher's F value was 1.46 (p = 0.05). This resulted in a non-significant effect; however, the effect size was medium ($\omega^2 = 0.10$) according to \citet{field2013discovering} conventions, suggesting a meaningful difference that may be detected with a larger sample size.

% In planning for a follow-up between-subjects study, a power analysis was conducted using the pwr package in R to estimate the necessary sample size to achieve a power of 0.80, assuming the same effect size and a significance level of 0.05. This power analysis indicated that approximately 30 (29.92) participants would be needed per group to achieve the desired statistical power, given the observed effect size from the preliminary study. 

% This estimate is based on the assumption that the effect size in the follow-up study would be similar to that observed in the preliminary study. Between studies can have lower power, depending on the true effect size, the variance of the data, and the design of the follow-up study. 

% Due to the widespread use of the UEQ average standard deviations and a procedure to estimate sample sizes are published~\cite{Schrepp2023-yf}. In comparison to the Benchmarks, our participants had low agreement in assessing the prototypes and a bigger sample may be preferred. For example, in order to achieve a 95\% confidence interval with a width of 0.04 (which can detect a 20\% difference in survey participants scoring at least 1 point higher), the required number of participants can be calculated using the average standard deviation of the UEQ across all prototypes and conditions. This yields a minimum required sample size of roughly 150 participants: $n > \left(\frac{2 \times 1.96 \times 1.23}{0.4}\right)^2 = 145.29$.



% \subsection{Further Statistical Tests}
% While the Trust Data Use and Trustworthy Content measures seem to exhibit differences for the Onboarding prototype, they appear to be nearly identical for the live view condition ($\omega_p^2 = 8.12 \times 10^{-3}$). This similarity might be attributed to the within-study design, where users could perceive that the underlying technology remains unchanged. Alternatively, it could be that the live visualization of the camera genuinely does not impact these measures. To gather evidence of these observations, a follow-up between-study analysis should conduct equivalence tests, such as a TOST (Two One-Sided Test), using meaningful equivalence bounds



==> fig_mockups.tex <==
\begin{figure*}[t]
      \centering
       \includegraphics[trim=34cm 7cm 79cm 25cm, clip=true, width=1.0\textwidth]{Figures/Mock-up.pdf}
\captionsetup{width=1.0\textwidth}   
\caption{Zoomed-in view of the Freeform board for designing the Mockups. These wireframes are similar to the final implemented prototype.}
      \Description{Zoomed-in view of the Freeform board for designing the Mockups. These wireframes are similar to the final implemented prototype.}
    \label{fig:Mockup}
\end{figure*}



==> fig_violins_liveview.tex <==



==> tab_reliability_analysis.tex <==
\begin{table}[ht]
\centering
\small
\begin{tabular}{|l|p{6.2cm}|c|c|c|}
\hline
\textbf{Scale} & \textbf{Items} & \textbf{Mean} & \textbf{SD} & \textbf{Cronbach's $\alpha$} \\ 
\hline
Pragmatic Quality & \makecell[l]{I think the technology and user interface is:\\ - obstructive:supportive \\ - complicated:easy \\- inefficient:efficient \\ - confusing:clear} & 1.3 & 1.2 & 0.875 \\
\hline
Hedonic Quality & \makecell[l]{I think the technology and user interface is: \\ - boring:exciting \\ - not interesting:interesting \\ - conventional:inventive \\ - usual:leading edge} & 1.29 & 1.3 & 0.932 \\
\hline

Trustworthy Content & \makecell[l]{In my opinion, the information and data \\provided by the product are:\\ - useless:useful \\ - implausible:plausible \\- untrustworthy:trustworthy \\- inaccurate:accurate} & 0.87 & 1.09 & 0.801 \\
\hline
Trust Data Use & \makecell[l]{Regarding the use of my personal information \\and data, the product is:\\ - insecure:secure \\ - untrustworthy:trustworthy \\- unreliable:reliable \\ - non-transparent:transparent} & 0.53 & 1.25 & 0.871 \\
\hline
Creepy & \makecell[l]{Strongly disagree:strongly agree:\\- I find this technology creepy. \\- This technology makes me feel uncomfortable. \\- The way this technology uses (personal) \\information is unsettling.} & -1.3 & 1.66 & 0.965 \\ 
\hline

\end{tabular}
\caption{Tect of suibcale items and scale reliability statistics (N=12).}
   \label{tab:scalereliability}
\end{table}

